Kinetic energy fluctuation-driven locomotor transitions on potential energy landscapes of beam obstacle traversal and self-righting

Despite contending with constraints imposed by the environment, morphology, and physiology, animals move well by physically interactingwith the environment to use and transition between modes such as running, climbing, and self-righting. By contrast, robots struggle to do so in real world. Understanding the principles of how locomotor transitions emerge from constrained physical interaction is necessary for robots to move robustly using similar strategies. Recent studies discovered that discoid cockroaches use and transition between diverse locomotor modes to traverse beams and self-right on ground. For both systems, animals probabilistically transitioned between modes via multiple pathways, while its self-propulsion created kinetic energy fluctuation. Here, we seek mechanistic explanations for these observations by adopting a physics-based approach that integrates biological and robotic studies. We discovered that animal and robot locomotor transitions during beam obstacle traversal and ground self-righting are barrier-crossing transitions on potential energy landscapes. Whereas animals and robot traversed stiff beams by rolling their body betweenbeam, they pushed across flimsy beams, suggesting a concept of terradynamic favorability where modes with easier physical interaction are more likely to occur. Robotic beam traversal revealed that, system state either remains in a favorable mode or transitions to one when energy fluctuation is comparable to the transition barrier. Robotic self-righting transitions occurred similarly and revealed that changing system parameters lowers barriers over which comparable fluctuation can induce transitions. Thetransitionsof animalsin both systems mostly occurred similarly, but sensory feedback may facilitate its beam traversal. Finally, we developed a method to measure animal movement across large spatiotemporal scales in a terrain treadmill.

==> ch0_acknowledgments/acknowledgments.tex <==
\chapter*{Acknowledgments}

I am deeply indebted grateful to my advisor, Prof. Chen Li, for accepting me into his group, the effort he put into training me on multiple fronts, and the kindness he has shown me over the years. Working with him since day 1 of Terradynamics Lab has been a rewarding experience. 

I would like to thank the Prof. Noah Cowan for all the advise, academic and otherwise, and his mentoring over the years. all Noah, Louis, Dr. C, Yannis, Avanti, Dr. Kim, Dr. Sudheer A. P., who introduced me to robotics; Prof. Subir Kumar Saha and Prof. Rajeevlochana Chittawadigi for their mentoring, advice, and support,  Sir, Mr. Rajendran Painghu, Ms. Bindu P.K for the amazing support and encouragement to a naive 17 year old me, Dr. Ravikrishna Menon for the training he offerred, Dr. Armand (DQE committee)

I thank members of Terradynamics Lab, past and present, for keeping it interesting conducive environment for research--Sean Gart for my constant questions in imaging, Rick Han for various help and advice throughougt projects, Tommy Mitchel for keeping it real, Qihan Xuan for his , Qiyuan Fu, Yaqing Wang, Allen Ren, Divya Ramesh.
(Students you supervised)

Funding

: Mike Bernard, Kevin Adams, Lorrie Dodd, Jordan Card, Ashley Moriarty, Rose Chase, Help was always given to Hopkins to those who asked for it. 

I thank Noah Cowan, Simon Sponberg, Jean Michel Mongeau, Kaushik Jayaram, Shai Revzen for the career advice they have given me. 

Friends within and outside Hopkins -- Arun Nair and Karuna Agarwal for their sage advice and , Radhika Rajaram for helping me navigate initial days, Anjali Nelliat , Stephanie Hao;  Weiqi Wang, Qiaozhi Wang, Ting Yung Fang for  Tommy Mitchel, Poojan Oza who has been an amazing roomate. Emanuel Chirayath, Prof.(!) Safvan Palathingal, and Nirmal Sabu for their camaraderie since our days as roommates at NIT.

Finally, I thanks my family: My parents Sadanandan and Poornima, for their unconditional love and support in pursuing my dreams. My grandmother Sarojini for her constant encouragement and prayers. My brother Rajat, who has often been the elder (and very likely the richer) one between us, Rupini Shukla, for her love and support over the past couple of years.

==> tables/e_table1.tex <==
\begin{table}[]
\begin{tabular}{|l|l|}
\hline
\textbf{Component}    & \textbf{Mass (g)} \\ \hline
Head                  & 13.4              \\ \hline
Leg rod               & 4.3               \\ \hline
Leg added mass        & 51.5              \\ \hline
Leg motor             & 28.6              \\ \hline
Two wings             & 57.4              \\ \hline
Two wing pitch motors & 56.0              \\ \hline
Two wing roll motors  & 48.8              \\ \hline
Total                 & 260.0             \\ \hline
\end{tabular}
\label{e_t1}
\end{table}

==> tables/e_table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{lllll}
\multicolumn{2}{l}{\textbf{Parameter}}                               & \textbf{Animal} & \textbf{Robot}        & \textbf{Ratio} \\
\multicolumn{2}{l}{Body length 2$a$ (mm)}                              & 53              & 260                   & 4.9            \\
\multicolumn{2}{l}{Body width 2$b$ (mm)}                               & 23              & 220                   & 9.6            \\
\multicolumn{2}{l}{Body thickness 2$c$ (mm)}                           & 8               & 43                    & 5.4            \\
\multicolumn{2}{l}{Mass attached to leg (g)}                         & 0.14            & 51.5                  & 368            \\
\multicolumn{2}{l}{Total mass $m$* (g)}                                & 2.84            & 260                   & 90             \\
\multicolumn{2}{l}{Density $\rho$ ($\times$10−3 g∙mm−3)}                         & 0.88            & 2.05                  & 2.3            \\
\multicolumn{2}{l}{Expected length scale factor ($(m/\rho)^{1/3}$)}            & 1.47            & 5.06                  & 3.4            \\
\multicolumn{2}{l}{Expected potential energy scale factor $m_{4/3}/\rho_{1/3}$} & 4.28            & 1306                  & 305            \\
\multicolumn{2}{l}{Maximum pitch potential energy barrier (mJ)}      & 0.58            & 282                   & 486            \\
\multicolumn{2}{l}{Maximum roll potential energy barrier (mJ)}       & 0.19            & 244                   & 1284           \\
\multirow{2}{*}{Froude number for leg flailing  $Fr$}  & Intact legs   & 0.37            & \multirow{2}{*}{0.78} & 2.1            \\
                                                     & Modified legs & 1.27            &                       & 0.61          
\end{tabular}
\label{e_t2}
\end{table}

==> tables/p_table2.tex <==

\clearpage
\begin{landscape}
\begin{table}[t!]
\centering
\caption{Torsional stiffness of our beams in comparison with natural obstacles.}

\begin{tabular}{ccccc}
Plant & Source & Flexural rigidity, \textit{EI} ($\mu$N$\cdot$m$^2$) & Length \textit{L} (m)& Torsional Stiffness \textit{K} (mN$\cdot$/rad)\\
\midrule
Katsura  	        & \citep{Bhosale2020}		&	4.4 - 11		&	0.07	&	0.06 - 0.16	\\
Red oak  			& \citep{Louf2018}           &	14.5 - 55.8		&	0.2		&	0.07 - 0.3	\\
\textit{K}1         & This study 	            &	-				&	-	 	&	0.1			\\
Yellow poplar 		& \citep{Louf2018}           &	19 - 124 		&	0.17 	&	0.1 - 0.7	\\
\textit{K}2         & This study		        &	-				&	-		&	0.2			\\
American sycamore   & \citep{Louf2018}           &	23.5 - 58.5		&	0.13	&	0.2 - 0.5	\\
Sugar maple 		& \citep{Louf2018}           &	29.8 - 144		&	0.1		&	0.3-1.4		\\
\textit{K}3         &This study		            &	-				&	-		&	0.7			\\
Sunflower 			&\citep{vogel1992a,Kurepin2007} &	73				&	0.07	&	1			\\
\textit{K}4         &This study		&	-				&	 -		&	1.7			\\
Red maple 			&\citep{vogel1992a,RedMaple_fl_2020}       &	194				&	0.076	&	2.5			\\
Quaking aspen 		&\citep{Niklas1991,NDTHandbook}       &	200				&	0.06	&	3.3			\\
Sweet gum 			&\citep{vogel1992a,Sweetgum_fl_2020}	    &   984				&	0.1		&	9.8			\\
\textit{K}5         &This study		            &	-				&	-		&	11.4		\\
Cucumber 			&\citep{vogel1992a,Blanco2005}&	8730			&	0.2		&	43.7 		\\

\bottomrule
\label{table:p_t1}
\end{tabular}
\end{table}
\noindent We surveyed literature of actual flexible terrain elements to assess how our beams compared. We approximated each terrain element as a cantilever beam. We then estimated torsional stiffness \textit{K} of the terrain element as \textit{K} $= \frac{EI}{L}$, where \textit{E} is Young’s modulus, \textit{I}  is the area moment of inertia of beam cross section,  and \textit{L} is the length of the cantilever beam. We obtained \textit{E}, \textit{I}, and \textit{L} from each study. We found that our beam obstacles are representative. In addition, because our energy landscape model is from first principles, the physical principles we discovered are likely general and apply beyond the stiffness range tested.

\end{landscape}
